ArabLegalEval: A Multitask Benchmark for Assessing Arabic Legal Knowledge in Large Language Models

The rapid advancements in Large Language Models (LLMs) have led to significant improvements in various natural language processing tasks. However, the evaluation of LLMs' legal knowledge, particularly in non-English languages such as Arabic, remains under-explored. To address this gap, we introduce ArabLegalEval, a multitask benchmark dataset for assessing the Arabic legal knowledge of LLMs. Inspired by the MMLU and LegalBench datasets, ArabLegalEval consists of multiple tasks sourced from Saudi legal documents and synthesized questions. In this work, we aim to analyze the capabilities required to solve legal problems in Arabic and benchmark the performance of state-of-the-art LLMs. We explore the impact of in-context learning and investigate various evaluation methods. Additionally, we explore workflows for generating questions with automatic validation to enhance the dataset's quality. We benchmark multilingual and Arabic-centric LLMs, such as GPT-4 and Jais, respectively. We also share our methodology for creating the dataset and validation, which can be generalized to other domains. We hope to accelerate AI research in the Arabic Legal domain by releasing the ArabLegalEval dataset and code: https://github.com/Thiqah/ArabLegalEval

==> latex/conclusion.tex <==
\section{Conclusion}


\hypertarget{limitations}{%
\subsubsection{Limitations}\label{limitations}}

\hypertarget{data-source-diversity}{%
\paragraph{Data Source Diversity}\label{data-source-diversity}}


\hypertarget{limitations-of-synthetic-data-generation}{%
\paragraph{Limitations of Synthetic Data
Generation}\label{limitations-of-synthetic-data-generation}}

\begin{itemize}
\tightlist
\item
  \textbf{Model Familiarity}: Judge models tend to prefer answers generated by themselves as pointed out by (Zheng et al. 2023) \cite{Zheng-et-al-judging}
\item
  \textbf{Quality Dependency}: The quality of the generated questions is
  limited by the capabilities of the model used. If the model has
  deficiencies, these will be reflected in the generated data.
\end{itemize}

\hypertarget{general-limitations-of-the-benchmark}{%
\paragraph{General Limitations of the
Benchmark}\label{general-limitations-of-the-benchmark}}

\begin{itemize}
\tightlist
\item
  \textbf{Dialect Limitations}: The dataset is primarily focused on
  Arabic Fusha, the standard dialect, and does not account for regional
  dialects.
\item
  \textbf{Limited Quantity}: The dataset includes 10,000 samples of
  synthetically generated or translated data and 1,357 questions from
  human-generated data, which have been filtered by human experts. While
  we sample the quality using Yamine's formula, the overall quantity may
  not be sufficient for comprehensive evaluation.
\item
  \textbf{Regional Bias}: Most of the data is derived from Saudi Arabian
  law, which, while generally applicable to other Arabic-speaking
  regions due to the inclusion of neutral legal contracts and user
  agreements, still introduces a regional bias.
\end{itemize}

\hypertarget{implications-of-these-limitations}{%
\paragraph{Implications of These
Limitations}\label{implications-of-these-limitations}}

The limitations highlighted above have several implications for the use
and evaluation of ArabLegalEval:

\begin{enumerate}
\def\labelenumi{\arabic{enumi}.}
\tightlist
\item
  \textbf{Generalizability}: The focus on Arabic Modern Standard Arabic (MSA) means that the
  benchmark may not fully capture the nuances of regional dialects,
  potentially limiting its applicability in contexts where these
  dialects are prevalent.
\item
  \textbf{Depth of Evaluation}: The limited quantity of data, especially
  the human-generated and filtered questions, may constrain the depth of
  evaluation and the ability to draw robust conclusions about model
  performance.
\item
  \textbf{Quality Control}: The reliance on synthetic data generation
  raises concerns about the consistency and accuracy of the questions,
  as the generated content is only as good as the models used to create
  it.
\item
  \textbf{Regional Focus}: While the benchmark includes some neutral
  legal content, the predominance of Saudi Arabian law could limit the
  benchmark's relevance in other legal contexts, particularly those with
  different legal frameworks.
\end{enumerate}

Despite these limitations, ArabLegalEval represents a significant step
forward in the evaluation of Arabic legal LLMs, providing a much-needed
benchmark for this under-explored area. By addressing these limitations
in future iterations, we aim to enhance the benchmark's applicability
and robustness, ultimately advancing the field of Arabic legal AI.

\subsection{Future work}
Even with state-of-the-art model, AI performance in the Arabic legal domain leaves a lot to be desired. In this paper, due to time constraints, the evaluation runs were not comprehensive enough to examine all Arabic LLMs, we aim to also test out the ability of pretrained models (non-instruct models) to solve MMLU tasks, as they may have an advantage over aligned models. There are also efforts to exploit the graph-like structure of legal documents and use graph traversial to retrieve relevant contexts for question answering and reasoning tasks, rather than using flat embedding-based retrieval.


==> latex/translation.tex <==



\subsection{Finding the best translation model}
Identifying the most suitable model is a critical step in obtaining a high-quality translated dataset. In our study, we evaluated three different machine translation models and GPT-4 Turbo to determine the best translator for a publicly available dataset with legal context. The dataset used in these experiments is the United Nations Parallel Corpus [1], which consists of United Nations documents in the six official UN languages: Arabic, Chinese, English, French, Russian, and Spanish. For the purpose of our research, we focused solely on the English and Arabic corpus. This choice was motivated by the unique challenges Arabic poses for machine translation especially in the legal domain. By using a dataset representative of real-world legal text, we can accurately assess the model’s performance in producing high-quality translations. The English and Arabic dataset in the United Nations Parallel Corpus comprises 20 million rows. However, to expedite the experimentation process, we utilized a subset of 14,000 examples from this dataset. This subset was used to evaluate the performance of the selected models without any preprocessing steps. The evaluation process involved assessing each model's translation quality based on Rouge metrics, Rouge stands for ``\textbf{Recall-Oriented Understudy for Gisting Evaluation}'' and it is a set of metrics used to measure the performance of machine generated text and commonly used in translation and summarization. Rouge score assesses the similarity between the machine-generated text and a reference text and is calculated by comparing the overlap of n-grams between the machine-generated text and the reference text. The score ranges from 0 to 1 with 1 indicating higher degree of similarity between texts.
In our evaluation, we employed three ROUGE metrics: ROUGE-1, ROUGE-2, and ROUGE-L, to assess the quality of the machine-generated translations against the reference translations. ROUGE-1 measures the overlap of unigrams (single words), providing a basic understanding of lexical similarity. ROUGE-2 measures the overlap of bigrams (two-word sequences), offering insights into contextual coherence. ROUGE-L measures the longest common subsequence (LCS), evaluating sentence-level structure similarity and fluency.
By comparing the results obtained from the different models, we aimed to identify the one that consistently produced the best translation from English to Arabic in the legal domain.The results of our experiments on this subset of data, without any prepossessing, are as in Table {}. We observed that Rouge-1 scores were consistently higher across all the models followed by the Rouge-L scores, and this indicates that the models performed better in capturing unigram overlap and the longest common subsequence between the machine-generated translations and the reference translations . Overall, Opus model outperformed the other models across all the metrics. The Opus model achieved a ROUGE-1 score of 0.52, a ROUGE-2 score of 0.3, and a ROUGE-L score of 0.51.


\begin{table}[]
\begin{tabular}{|c|c|c|c|}
\hline
Model                      & Rouge-1             & Rouge-2             & Rouge-L             \\ \hline
Azure Translation Services & 0.446208796042216   & 0.24281469776438544 & 0.43513631898755084 \\ \hline
Google Translation API     & 0.40874384087024945 & 0.2077645187878664  & 0.3990715620486186  \\ \hline
Opus MT                    & 0.5194083323372131  & 0.30834225296184536 & 0.5092002777657184  \\ \hline
GPT 4 Turbo                & 0.3279289607952094  & 0.13866838050577932 & 0.3167879369113815  \\ \hline
\end{tabular}
\caption{Machine Translation Results}
\label{tab:my-table}
\end{table}

These findings offer important insights into each model's performance and establish a basis for selecting the best translator for our main task: translating legal datasets from English to Arabic. The results we obtained were not definitive in the model selection process due to several issues observed in the data, which could directly impact the final outcomes. Some of these issues include:

\begin{enumerate}
\item Incomplete text
\item Unclean text (containing random symbols)
\item Text orientation is from left to right
\item incorrect mapping between English and Arabic text
\item Missing Arabic Text from the Arabic reference text
\end{enumerate}

Despite the limitations in the dataset, from our experiment we found that Opus was the best machine translator to translate the UN dataset. 

The chosen model will be used to translate the four datasets selected from LegalBench, enabling us to evaluate the capabilities of Large Language Models in understanding and interpreting legal clauses and contracts in the Arabic language.

[[Example of some of the issues?]]

\subsubsection{Consumer Contracts QA}
This task assess the legal skill of contract interpretation in the context of consumer contracts. This task requires analysis of clauses within terms of service agreements and determine whether they create specific rights or obligations for the parties involved. It demonstrates the LLMs ability to interpret and understand the legal implications of these contractual provisions.

\subsubsection{\textit{Contracts QA}}
This task tests the LLMs ability to determine whether contractual clauses cover specific types of content. 
The LLM needs to analyze the language of each contractual clause and determine if it pertains to the specific content types in question. This task assesses the LLM's capability to comprehend and categorize legal language, even when faced with clause types that are not explicitly exemplified in the prompt.

\subsubsection{\textit{Privacy Policy QA}}

This task assesses LLMs ability to determine the relevance of privacy policy clauses to specific questions. The LLM must classify the question-clause pair as either Relevant'' or Irrelevant'' based on whether the clause contains sufficient information to answer the question. This task evaluates the LLM's capability to understand and interpret legal language in privacy policies, as well as its ability to identify the relevance of specific clauses to given questions. This task assesses the LLM's comprehension of legal text and its capacity to extract pertinent information from privacy policies.
\subsubsection{\textit{Privacy Policy Entailment}}
Given a privacy policy clause and description, the objective is to assess whether the description accurately represents the privacy policy clause. The LLM receives a clause from a privacy policy and its description. The LLM must then classify the description as either Correct'' or Incorrect'' based on the clause's content.

\subsection{Translation Methodology}
To ensure the highest translation quality, we employed the three models from our initial experiments to translate the ``Consumer Contract QA'' dataset. We conducted a manual inspection of the overall results and, to further enhance the quality assessment, engaged both GPT-4 and legal experts as evaluators for the translated content.
\subsubsection{GPT-4 Evaluation}
We tasked GPT-4 with evaluating a sample of the translated text alongside the original text, asking it to rate the translation quality on a scale from 1 to 5. Interestingly, GPT-4 consistently rated the translations as either 4 or 5 out of 5, indicating a high level of perceived quality.
Examples of the evaluation: 

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{latex//assets/GPT4_Evaluation.png}
    \caption{GPT 4 feedback on one of the Examples}
    \label{fig:enter-label}
\end{figure}
\subsubsection{Human Evaluation}
We selected five examples from the translated texts, each consisting of a contract text and a corresponding question. To evaluate the performance of the three translation models—Azure Translation Services, Google API Services, and Opus MT—we asked legal experts to assess each contract and question separately. The experts provided scores for each model's translation quality.
The overall scores for all three models were relatively close, but Opus MT achieved the highest score among them:
\begin{itemize}
\item Google API Translation: Average score of 3.3 out of 5
\item Azure Translation Services: Average score of 3.56 out of 5
\item Opus MT: Average score of 4 out of 5
\end{itemize}
In addition to the overall scores, we asked the experts to rank the best model for each example. Opus MT was chosen as the best model 60\% of the time, while Azure Translation Services was selected 40\% of the time. Interestingly, Google API Translation was never selected as the best model for any of the examples.

These results suggest that while all three models performed reasonably well, Opus MT demonstrated superior translation quality for the given legal texts and questions, as determined by the expert evaluations.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{Sample TranslatiedData.png}
    \caption{Sample of the Translated Data}
    \label{fig:enter-label}
\end{figure}

\subsection {Running the Benchmarks and Analysis }
\subsubsection{ Experiments Setup}

In total, we carried out 96 unique experiments. For the Contract QA and Consumer Contract datasets, we utilized the entire testing data in our experiments. However, for the larger datasets, we selected a representative sample to ensure efficient processing and analysis. We crafted a customized prompt for each technique and ran the benchmark on all the models using the four approaches mentioned above.

\begin{itemize}
\item Zero-Shot Learning with Simple Prompts
\item Zero-Shot Learning with Detailed Instructions
\item One-Shot Learning
\item Few Shot Learning
\end{itemize}

[will add Example Prompts] 

In total, we carried out 96 unique experiments. For the Contract QA and Consumer Contract datasets, we utilized the entire testing data in our experiments. However, for the larger datasets, we selected a representative sample to ensure efficient processing and analysis. We crafted a customized prompt for each technique and ran the benchmark on all the models using the four approaches mentioned above.

\subsubsection{Results Analysis}

The results on the evaluated datasets are as follows:
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{latex/image.png}
    \caption{Will convert this into better visual}
    \label{fig:enter-label}
\end{figure}






